The Abstract Machinery of Interaction (Long Version)

This paper revisits the Interaction Abstract Machine (IAM), a machine based on Girard's Geometry of Interaction, introduced by Mackie and Danos & Regnier. It is an unusual machine, not relying on environments, presented on linear logic proof nets, and whose soundness proof is convoluted and passes through various other formalisms. Here we provide a new direct proof of its correctness, based on a variant of Sands's improvements, a natural notion of bisimulation. Moreover, our proof is carried out on a new presentation of the IAM, defined as a machine acting directly on $\lambda$-terms, rather than on linear logic proof nets.

==> proofs/good-invariant-proof.tex <==
% !TEX root = ../main.tex
\begin{proof}
  Let $\state = \dstate{\tm}{\ctxhole}{\resm^h}{\stempty} \toiam^k \statetwo$. By
  induction on $k$. For $k=0$ there is nothing to prove because the state has no tape nor log tests. Then suppose
  $\state\toiam^{k-1}\statethree\toiam\statetwo$. By \ih, $\statethree
  = \nopolstate{\tmtwo}{\ctx}{\stme}{\ste}{\pol}$ is exhaustible, and with
  this hypothesis we need to conclude that $\statetwo$ is exhaustible, too.
  There are many cases to take into account, depending on the transition used to
  move from $\statethree$ to $\statetwo$.
  
  First,
  suppose that $\pol = \downp$. Cases of $\statethree\toiam\statetwo$:
  \begin{enumerate}
  \item
    \emph{Application}, \ie\ $\tmtwo = \tmthree\tmfour$ and
	\begin{center}$
    	   \dstate{ \tmthree\tmfour }{ \ctx }{ \stme }{ \ste } 
	   \iamdap 
	   \dstate{ \tmthree }{ \ctxp{\ctxhole\tmfour} }{ \resm\cons \stme }{ \ste } = \statetwo.
	 $\end{center}
	 We have to show that the obtained state $\statetwo$ is
         exhaustible. For log tests, it follows from
         \reflemmap{outer-inv}{three} and the \ih:
         $\statethree$ is a head translation of $\statetwo$, and the
         lemma states that they have the same log tests, which are
         exhaustible because $\statethree$ is exhaustible by \ih
		
	 For the tape test, consider the decomposition $\stme =
         \resm^k\cons\exps\cons\stmetwo$.
            Then the tape test
           $\statethree_\exps$ of $\statethree$ reduces to
           $\statetwo_\exps$:
	   	\begin{center}$
           \statethree_\exps = \dstate{ \tmthree\tmfour }{ \ctx }{ 
           \resm^k\cons\exps\cons\stmetwo }{ \ste } \iamuapltwo 
           \dstate{\tmthree}{ 
           \ctxp{\ctxhole\tmfour} }{ \resm^{k+1}\cons\exps\cons\stmetwo}{ \ste 
           } = 
           \statetwo_\exps
           $\end{center}
           By \ih, $\statethree$ is exhaustible, then
           $\statethree_\exps$ evolves to an exhaustible state
           surrounding  $\exps$, but for the tape being $\stmetwo$, call it 
           $\statefour_\exps$.
           The IAM is deterministic,
           so $\statetwo_\exps$ itself
           reduces to $\statefour_\exps$.
	 \item \emph{Abstraction 1}, \ie\ $\tmtwo=\la\var\tmthree$ and 
	 $\stme=\resm\cdot\stmetwo$. This case is equivalent to the previous one.
	% VARIABLE DOWN
    \item \emph{Variable bound by an abstraction}, \ie\ $\tmtwo = \var$ and
      	\begin{center}$\begin{array}{lll}
      \statethree = & \dstate{ \var }{ \ctxp{\l\var.\ctxtwo_n} }{ \stme }{ \expsn\cdot\ste } 
      \\
      \iamdvar &
      \ustate{ \l\var.\ctxtwo_n\ctxholep\var}{ \ctx }{ (\var,\l\var.\ctxtwo_n,\expsn)\cdot\stme }{ \ste } = \statetwo
      	\end{array}$\end{center}
      The proof that $\statetwo$ is exhaustible is divided in two parts:
      \begin{enumerate}
      \item
        \emph{Log testing}. By \reflemmap{outer-inv}{four}, all log tests of $\statetwo$
        are also log tests of $\statethree$. Since the latter is
        exhausible by \ih, then all the log tests of
        $\statetwo$ are successful.
        %Suppose that the level of $\ctx$ is
        %$i$. By \reflemmap{outer-inv}{four}, $\outs\statetwo = \outsi
        %     {i-1} \statethree$. By \ih, $\statethree$ is exhaustible,
        %     and so by \reflemma{recursive-good} $\outsi {i-1}
        %     \statethree$ is exhaustible.		
      \item \emph{Tape testing}.
        Let us consider the decomposition $\stme =
        \resm^k\cons\exps\cons\stmetwo$. Observe that
          by definition $\statetwo_\exps$, the tape test of $\statetwo$ has the 
          following property:
      	\begin{center}$\begin{array}{lll}
          \statetwo_\exps = & \dstate{ \l\var.\ctxtwo_n\ctxholep\var}{ \ctx }{ 
          (\var,\l\var.\ctxtwo_n,\expsn)\cdot\stme}{ \ste }
          \\
          \iamdlamtwo & \ustate{ \var}{ \ctxp{\l\var.\ctxtwo_n} }{ \stme}{ 
          \expsn\cons\ste} = \statethree^\bot
      	\end{array}$\end{center}
          where $\statethree^\bot$ is trivially surrounding $\exps$, but for 
          the tape $\stme$.
          Moreover, by \ih, $\statethree$ is exhaustible, a property
          which is easily transferred to $\statethree^\bot$: the log tests are 
          the same by \reflemmap{outer-inv}{one}, while $\statethree^\bot$ 
          satisfies tape testing, because the test state does not depend on the 
          polarity.
	
	\end{enumerate}
	
	% ABSTRACTION DOWN
    \item
      \emph{Abstraction 2}, \ie\ $\tmtwo = \l\var.\ctxtwo_n\ctxholep{\var}$ and
      	\begin{center}$\begin{array}{lll}
      \statethree = &
      \dstate{ \l\var.\ctxtwo_n\ctxholep{\var} }{ \ctx }{
        (\var,\la\var\ctxtwo_n,\stetwo)\cons\stme }{ \ste }
      \\
      \iamdlamtwo & \ustate{ \var}{ \ctxp{\la\var\ctxtwo_n} }{ \stme }{
        \stetwo \cons\ste } = \statetwo
            	\end{array}$\end{center}
      \begin{enumerate}
      \item
        \emph{Log testing}.  Let $\exps =
        (\var,\ctxp{\la\var\ctxtwo_n},\stetwo)$ and note that the tape tests of $\statethree$ of focus $\exps$ does the following transition:
      	\begin{center}$\begin{array}{lll}
        \statethree_\exps = &
        \dstate{ \l\var.\ctxtwo_n\ctxholep{\var} }{ \ctx }{ 
        (\var,\la\var\ctxtwo_n,\stetwo) }{ 
        \ste } 
        \\
	\iamdlamtwo &
	\ustate{ \var}{ \ctxp{\la\var\ctxtwo_n} }{ \stempty}{ \stetwo \cons\ste }  = \statetwo_\stempty
              	\end{array}$\end{center}
        Now, $\statetwo_\stempty$ surrounds $\exps$ and thus, by \ih (tape testing of $\statethree$), $\statetwo_\stempty$ is exhaustible. By \reflemmap{outer-inv}{two}, $\statetwo_\stempty$ and $\statetwo$ have the same log tests, so log testing for $\statetwo$ holds because it does for $\statetwo_\stempty$.
      \item
        \emph{Tape testing}. Note that $\statethree_\exps$, the tape 
        test of $\statethree$ corresponds to $\statethree$. Thus by \ih\ it 
        reduces in the following way:
      	\begin{center}$\begin{array}{lll}
      		\statethree=\statethree_\exps = &
      		\dstate{ \l\var.\ctxtwo_n\ctxholep{\var} }{ \ctx }{
      			(\var,\la\var\ctxtwo_n,\stetwo)\cons\stme }{ \ste }
      		\\
      		\toiam^* & \ustate{ \var}{ \ctxp{\la\var\ctxtwo_n} }{ \stme }{
      			\stetwo \cons\ste } = \state^\star \in\exstates
      		\end{array}$\end{center}
      	Hence, since $\state_\star=\statetwo$, also $\statetwo$ is exhaustible.
      \end{enumerate}
      
      \item \emph{Explicit Substitution}, \ie $\tmtwo = \tmthree\esub\var\tmfour$ and
      	\begin{center}$
	    \statethree = \dstate{ \tmthree\esub\var\tmfour }{ \ctx }{ \stme }{ \ste } 
    \iamdes 
    \dstate{ \tmthree }{ \ctxp{\ctxhole\esub\var\tmfour} }{ \stme }{ \ste } = \statetwo
    $\end{center}
 For log testing, it follows from
         \reflemmap{outer-inv}{three} and the \ih:
         $\statethree$ is a head translation of $\statetwo$, and the
         lemma states that they have the same log tests, which are
         exhaustible because $\statethree$ is exhaustible by \ih
		
	 For tape testing it goes exactly as the application case. We spell it out anyway. Consider a decomposition $\stme =
         \resm^k\cons\exps\cons\stmetwo$. Note that the tape test
           $\statethree_\exps$ of $\statethree$ reduces to
           $\statetwo_\exps$:
      	\begin{center}$\begin{array}{lll}
           \statethree_\exps = & \dstate{ \tmthree\esub\var\tmfour }{ \ctx }{ 
           \resm^k\cons\exps\cons\stmetwo }{ \ste } 
           \\
           \iamdes & \dstate{\tmthree}{ \ctxp{\ctxhole\esub\var\tmfour} }{ 
           \resm^k\cons\exps\cons\stmetwo}{ \ste } = \statetwo_\exps
              	\end{array}$\end{center}
           Again, we then proceed as usual, exploiting the determinism of
          the $\IAM$ and the \ih


	\item \emph{Variable bound by an explicit substitution}, \ie $\tmtwo = \var$ and
	\begin{center}$\begin{array}{lll}
	\statethree = &\dstate{ \var }{ \ctxp{\ctxtwo_n\esub\var\tmthree} }{ \stme }{ \expsn\cdot\ste } 
	\\
	 \iamdvartwo&
	\dstate{ \tmthree }{ \ctxp{\ctxtwo_n\ctxholep\var\esub\var\ctxhole} }{ \stme }{ (\var,\ctxtwo_n\esub\var\tmthree,\expsn)\cdot\ste } = \statetwo
	\end{array}$\end{center}
		\begin{enumerate}
			\item \emph{Log testing}: let $\exps \defeq (\var, \ctxtwo_n\esub\var\tmthree,\expsn)$ and $m = \size{\exps\cdot\ste}$. The $m$-log test of $\statetwo$ is 
				\begin{center}
				$\outsi{m}{\state} = \ustate{ \tmthree }{ \ctxp{\ctxtwo_n\ctxholep\var\esub\var\ctxhole} }{ \epsilon }{ (\var,\ctxtwo_n\esub\var\tmthree,\expsn)\cdot\ste }$
				\end{center}
			which makes a transition
				\begin{center}
				$\iamuestwo \ustate{ \var }{ \ctxp{\ctxtwo_n\esub\var\tmthree} }{ \epsilon }{ \expsn\cdot\ste } = (\statethree_\epsilon)^\bot$
				\end{center}
			that is a state surrounding $\exps$, as required by log testing. We have to prove that $(\statethree_\epsilon)^\bot$ is exhaustible. Tape testing is trivial, because the tape is empty. Log testing follows from the \ih\ and the fact that $(\statethree_\epsilon)^\bot$ is $\statethree$ with reversed direction and without the tape, and so by \reflemmap{outer-inv}{one} and \reflemmap{outer-inv}{two} they have the same log tests.
			
			Note that the $i$-log tests of $\statetwo$ for $i<m$ are the $i$-log tests of $\statetwo$ (\reflemmap{outer-inv}{four}), and so they satisfy the log testing clause by the \ih
			
			\item \emph{Tape testing}:  it goes exactly as in the previous 
			ordinary cases. We spell it out anyway. Consider a decomposition 
			$\stme =
			\resm^k\cons\exps\cons\stmetwo$.
            Note that the
           corresponding tape test
           $\statethree_\exps$ of $\statethree$ reduces to
           $\statetwo_\exps$, the tape test of $\statetwo$:
	   	\begin{center}$\begin{array}{lll}
		\statethree_\exps = &
           \dstate{ \var }{ \ctxp{\ctxtwo_n\esub\var\tmthree} }{ \stmetwo\cons\exps }{ \expsn\cdot\ste } 
           \\
	\iamdvartwo &
	\dstate{ \tmthree }{ \ctxp{\ctxtwo_n\ctxholep\var\esub\var\ctxhole} }{ \stmetwo\cons\exps }{ (\var,\ctxtwo_n\esub\var\tmthree,\expsn)\cdot\ste }   =\statetwo_\exps
	              	\end{array}$\end{center}
           Again, we then proceed as usual, exploiting the determinism of
          the $\IAM$ and the \ih.

      	\end{enumerate}
      \end{enumerate}
	%%
	%% UP CASES
	%%
        Now, suppose that $\pol = \upp$. Cases of
        $\statethree\toiam\statetwo$:
	\begin{enumerate}
		% UP - FROM APPLICATION LEFT
		\item \emph{Coming from the left of an application}, \ie\ $\ctx = \ctxtwop{\ctxhole \tmthree}$ and 
		  	\begin{center}$
                  \statethree = \ustate{ \tmtwo }{ \ctxtwop{\ctxhole\tmthree} }{ \exps\cdot\stme }{ \ste } 
                  \iamuaplone 
                  \dstate{ \tmthree }{ \ctxtwop{\tmtwo\ctxhole} }{ \stme }{ \exps\cdot\ste } = \statetwo.
                  $\end{center}
	          The proof that $\statetwo$ is exhaustible is divided in two parts:
	          \begin{enumerate}
		  \item
                    \emph{Log testing}. The log tests of
                    $\statetwo$ are those of $\statethree$ plus\\
                    $\ustate{ \tmthree }{ \ctxtwop{\tmtwo\ctxhole} }{ 
\epsilon}{ \exps\cdot\ste }$.
                    The former are fine because of the \ih, while
                    about the latter, observe that
                    $\ustate{ \tmthree }{ \ctxtwop{\tmtwo\ctxhole} }{ 
\epsilon}{ \exps\cdot\ste }$
                    evolves to $\dstate{ \tmtwo }{ \ctxtwop{\ctxhole\tmthree} 
                    }{ \exps }{ \ste }$
                    which is the tape test of $\statethree$, but for the 
suffix 
                    $\stme$ of the tape. The thesis
                    easily follows by \ih
		
		\item \emph{Tape testing}.
                    Let us consider a decomposition 
                    $\stme=\resm^k\cdot(\var,\ctxthree,\stetwo)\cdot\stmetwo$ 
                    and $\exps=(\vartwo,\ctxfour,\stethree)$. 
                    Note that the by \ih
				   	\begin{center}$\begin{array}{lll}
                      \statethree_\exps = &\dstate{ \tmtwo }{ 
                      \ctxtwop{\ctxhole\tmthree} }{ 
                      \exps\cdot\resm^k\cdot(\var,\ctxthree,\stetwo) 
                      \cdot\stmetwo}{ \ste } 
                      \\
                      \toiam^* &
		      \ustate{ \vartwo}{ \ctxfour_n\ctxholep\ctxfour }{ 
		      \resm^k\cdot(\var,\ctxthree,\stetwo)\cdot\stmetwo }{ 
		      \stethree\cdot\stethree_n }=\statethree_{\vartwo\upp}
	              	\end{array}$\end{center}
	              and then
	              \begin{center}$\begin{array}{lll}
	              	\statethree_{\vartwo\downp}=&\dstate{ \vartwo}{ 
	              	\ctxfour_n\ctxholep\ctxfour }{ 
	              		\resm^k\cdot(\var,\ctxthree,\stetwo)\cdot\stmetwo }{ 
	              		\stethree\cdot\stethree_n }
	              	\\
	              	\toiam^* &
	              	\ustate{ \var}{ \ctxthree_m\ctxholep\ctxthree }{ 
	              		\stmetwo }{ 
	              		\stetwo\cdot\stetwo_m }=\statethree_{\var\upp}
	              	\end{array}$\end{center}
                      By reversibility we have either                       
                      \begin{center}
                      	$\statethree_{\vartwo,\downp}\toiam^* 
                      	\statethree\toiam^* 
                      	\statethree_{\var\upp}$
                      	\end{center}
                      	or
                      	\begin{center}
                      		$\statethree_{\vartwo,\downp}\toiam^* 
                      		\statethree_{\var\upp}\toiam^*\statethree $
                      	\end{center}
                      	The second case is impossible since the logged position 
                      	$(\var,E,\stetwo)$ would be available on the tape both 
                      	before and after $\state_{\var\upp}''$, contradicting 
                      	the acyclicity.
                      	This concludes the proof of this case since 
                      	$\statethree\toiam\statetwo$.
		      %By \ih, $\statethree$ is exhaustible, then
                      %$\statethree_\exps
                      %\toiam^*\ustate{\tmtwo}{\ctxtwo}{\stempty}{\stetwo}=:
                      %\state_{\stempty}$ for some
                      %$\tmtwo,\ctxtwo,\stetwo$, with
                      %$\state_{\stempty}$ exhaustible. The IAM is
                      %deterministic, so $\statethree_\exps
                      %\iamuaplone\statetwo_\exps$ and
                      %$\statethree_\exps\toiam^*\state_{\stempty}$
                      %imply
                      %$\statetwo_\exps\toiam^*\state_{\stempty}$.
		    
	          \end{enumerate}
	          
			% UP - FROM APPLICATION RIGHT
		\item \emph{Coming from the right of an application}, \ie\ $\ctx = \ctxtwop{\tmthree \ctxhole}$ and 
						   	\begin{center}$    \statethree = \ustate{ \tmtwo }{ \ctxtwop{\tmthree\ctxhole} }{ \stme }{ \exps\cdot\ste }
                  \iamuapr 
                  \dstate{ \tmthree }{ \ctxtwop{\ctxhole\tmtwo} }{ \exps\cdot\stme }{ \ste } = \statetwo.
                  $\end{center}
	          The proof that $\statetwo$ is exhaustible is divided in two parts:
	          \begin{enumerate}
		  \item
                    \emph{Log testing}:
                    the log tests of $\statetwo$
                    are among the log tests of $\statethree$,
                    so log testing follows from \ih
                    %Note that $\statetwo$
                    %is almost the log test $\outs\statethree$ of
                    %$\statethree$: the only difference is that
                    %$\statetwo$ concatenates $\stme$ after $\exps$ in
                    %the tape. Now, note that (if $\outs\statetwo$
                    %is defined then) $\outs\statetwo = \outs {\outs
                    %  \statethree}$ because the log test does not
                    %depend on the tape, by
                    %\reflemmap{outer-inv}{four}.2. By exhaustibleness
                    %of $\statethree$ (\ih) and
                    %\reflemma{recursive-good}, $\outs {\outs
                    %  \statethree}$ is exhaustible.		
		  \item \emph{Tape testing}. The state to be proven exhaustible 
                    is                      
                      $$\statetwo_\exps = \dstate{ \tmthree }{
                        \ctxtwop{\ctxhole\tmtwo} }{ \exps\cdot\stme }{ \ste }$$
                      Now, note that the log test $\outsi{\size{\exps\cdot\ste}}\statethree$ of $\statethree$ reduces in one step to $\statetwo_\exps$:
				   	\begin{center}$\begin{array}{rll}
                      \outsi{\size{\exps\cdot\ste}}\statethree = & \ustate{ \tmtwo }{ \ctxtwop{\tmthree\ctxhole} }{ \epsilon}{ \exps\cdot\ste } 
                      \\
                      \iamuapr &
                      \dstate{ \tmthree }{
                        \ctxtwop{\ctxhole\tmtwo} }{ \exps }{ \ste }
	              	\end{array}$\end{center}
                      By log testing for $\statethree$, there is a state 
                      $q_\exps$ surrounding $\exps$ such that 
                      $\outsi{\size{\exps\cdot\ste}}\statethree \toiam^* 
                      q_\exps$. By determinism of the IAM, and \emph{pumping} 
                      $\stme$ on the tape one can conclude.
                      %We have to prove tape testing for the test
                      %state $$\statetwo_\exps = \dstate{ \tmthree }{
                      %  \ctxtwop{\ctxhole\tmtwo} }{ \exps }{ \ste }$$
                      %Note that $\statetwo_\exps$ is the log test
                      %of $\statethree$, which is exhaustible because
                      %$\statethree$ is exhaustible by \ih Since
                      %$\statetwo_\exps$ is its own test state, being
                      %exhaustible implies that it verifies IO
                      %decomposition.		      
		
	\end{enumerate}

\item \emph{Explicit Substitution}
\begin{center}$\statethree = \ustate{ \tmtwo }{ \ctxp{\ctxhole\esub\var\tmthree} }{ \stme }{ \ste } 
	\iamues 
	\ustate{ \tmtwo\esub\var\tmthree }{ \ctx }{ \stme }{ \ste } = \statetwo
$\end{center}
\begin{enumerate}
		\item \emph{Log testing}: by \reflemmap{outer-inv}{three} (head translation), the log tests of $\statetwo$ are log tests of $\statethree$, which satisfy log testing by the \ih
	
	\item \emph{Tape testing}: it goes exactly as for the other ordinary cases.
	\end{enumerate}
	
\item \emph{Coming from inside an explicit substitution}:
\begin{center}$\begin{array}{rll}
\statethree = & \ustate{ \tmtwo }{ \ctxp{\ctxtwop\var\esub\var\ctxhole} }{ \stme }{ (\var, \ctxtwo[\var\leftarrow\tmtwo],\stetwo)\cdot\ste } 
\\
	\iamuestwo &
	\ustate{ \var }{ \ctxp{\ctxtwo[\var\leftarrow\tmtwo]} }{ \stme }{ \stetwo\cdot\ste } = \statetwo
\end{array}$\end{center}
	\begin{enumerate}
		\item \emph{Log testing}: by \ih, $\statethree$ is exhaustible, and its $\size\ste +1$-log test evolves to 
		\begin{center}$\begin{array}{rll}
		\outsi{\size\ste +1}\statethree = & \ustate{ \tmtwo }{ \ctxp{\ctxtwop\var\esub\var\ctxhole} }{ \epsilon }{ (\var, \ctxtwo[\var\leftarrow\tmtwo],\stetwo)\cdot\ste } 
		\\
	\iamuestwo &
	\ustate{ \var }{ \ctxp{\ctxtwo[\var\leftarrow\tmtwo]} }{ \epsilon }{ \stetwo\cdot\ste } = \statetwo_\epsilon
	   	\end{array}$\end{center}
		which is exhaustible. By \reflemmap{outer-inv}{two}, $\statetwo_\epsilon$ and $\statetwo$ have the same log tests, which are then successful.
	
	\item \emph{Tape testing}: since the tape is unaffected by the transition, this case goes exactly as the other ordinary ones.
	\end{enumerate}		
	\end{enumerate}
\end{proof}

